Forward Modeling for Partial Observation Strategy Games - A StarCraft Defogger

We formulate the problem of defogging as state estimation and future state prediction from previous, partial observations in the context of real-time strategy games. We propose to employ encoder-decoder neural networks for this task, and introduce proxy tasks and baselines for evaluation to assess their ability of capturing basic game rules and high-level dynamics. By combining convolutional neural networks and recurrent networks, we exploit spatial and sequential correlations and train well-performing models on a large dataset of human games of StarCraft: Brood War. Finally, we demonstrate the relevance of our models to downstream tasks by applying them for enemy unit prediction in a state-of-the-art, rule-based StarCraft bot. We observe improvements in win rates against several strong community bots.

==> tikz/fancy_figure.tex <==
\begin{figure}[!ht]
\centering
\tdplotsetmaincoords{60}{125}
\newcommand{\viewa}{35} % this is 125 - 90
\newcommand{\viewb}{30} % this is 90 - 60
\begin{tikzpicture}
		[tdplot_main_coords,
			cube/.style={ultra thick,black},
			grid/.style={thick,red, opacity=0.65},
			axis/.style={->,blue,thick}]

      \foreach \x in {-3,-2,...,3}
      \foreach \y in {-3,-2,...,3}
      {
        \draw[grid] (\x,-3) -- (\x,3);
        \draw[grid] (-3,\y) -- (3,\y);
      }
      \def\mapsquare{(-3,-3,0)--(-3,3,0)--(3, 3, 0)--(3, -3, 0)--cycle}
      \begin{scope}
        \clip \mapsquare;
        % the picture
        \node[inner sep=0pt, opacity=0.65, cm={cos(\viewa),-sin(\viewa)*sin(\viewb), sin(\viewa),cos(\viewa)*sin(\viewb), (0,0)}] (map){\includegraphics[width=6cm]{tikz/map.jpg}};
      \end{scope}

      %% FIRST COLUMN
      % draw the top and bottom of the cube
      \coordinate (center1) at (2,-2,0);
      \coordinate (A) at ($(center1) + (-1,-1,0)$);
      \coordinate (B) at ($(center1) + (-1,1,0)$);
      \coordinate (C) at ($(center1) + (1,1,0)$);
      \coordinate (D) at ($(center1) + (1,-1,0)$);
      \coordinate (A2) at ($(center1) + (-0.5,-0.5,2)$);
      \coordinate (B2) at ($(center1) + (-0.5,0.5,2)$);
      \coordinate (C2) at ($(center1) + (0.5,0.5,2)$);
      \coordinate (D2) at ($(center1) + (0.5,-0.5,2)$);
      \draw[cube] (A) -- (B) -- (C) -- (D) -- cycle;
      \draw[cube] (A2) -- (B2) -- (C2) -- (D2) -- cycle;

      
      % draw the edges of the cube
      \draw[cube] (A) -- (A2);
      \draw[cube] (B) -- (B2);
      \draw[cube] (C) -- (C2);
      \draw[cube] (D) -- (D2);
	
      \draw[ultra thick,->] ($(0,0,2) + (center1) $)-- ($(0,0,3)  + (center1)$) node[above, draw, circle,yslant=-0.45](lstm){LSTM};
      \draw[ultra thick,->] (lstm.north) -- ($(0,0,6)  + (center1)$) ;
      \coordinate (bA) at ($(center1) + (-0.5,-0.5,6)$);
      \coordinate (bB) at ($(center1) + (-0.5,0.5,6)$);
      \coordinate (bC) at ($(center1) + (0.5,0.5,6)$);
      \coordinate (bD) at ($(center1) + (0.5,-0.5,6)$);
      \coordinate (bA2) at ($(center1) + (-1,-1,8)$);
      \coordinate (bB2) at ($(center1) + (-1,1,8)$);
      \coordinate (bC2) at ($(center1) + (1,1,8)$);
      \coordinate (bD2) at ($(center1) + (1,-1,8)$);
      \draw[cube] (bA) -- (bB) -- (bC) -- (bD) -- cycle;
      \draw[cube] (bA2) -- (bB2) -- (bC2) -- (bD2) -- cycle;
      \draw[cube] (bA) -- (bA2);
      \draw[cube] (bB) -- (bB2);
      \draw[cube] (bC) -- (bC2);
      \draw[cube] (bD) -- (bD2);

      %% SECOND COLUMN
      \coordinate (center2) at (-2,0,0);
      \coordinate (sA) at ($(center2) + (-1,-1,0)$);
      \coordinate (sB) at ($(center2) + (-1,1,0)$);
      \coordinate (sC) at ($(center2) + (1,1,0)$);
      \coordinate (sD) at ($(center2) + (1,-1,0)$);
      \coordinate (sA2) at ($(center2) + (-0.5,-0.5,2)$);
      \coordinate (sB2) at ($(center2) + (-0.5,0.5,2)$);
      \coordinate (sC2) at ($(center2) + (0.5,0.5,2)$);
      \coordinate (sD2) at ($(center2) + (0.5,-0.5,2)$);
      \draw[cube] (sA) -- (sB) -- (sC) -- (sD) -- cycle;
      \draw[cube] (sA2) -- (sB2) -- (sC2) -- (sD2) -- cycle;
      
      % draw the edges of the cube
      \draw[cube] (sA) -- (sA2);
      \draw[cube] (sB) -- (sB2);
      \draw[cube] (sC) -- (sC2);
      \draw[cube] (sD) -- (sD2);
	
      \draw[ultra thick,->] ($(0,0,2) + (center2) $)-- ($(0,0,3)  + (center2)$) node[above, draw, circle,yslant=-0.45](lstm){LSTM};
      \draw[ultra thick,->] (lstm.north) -- ($(0,0,6)  + (center2)$) ;
      \coordinate (sbA) at ($(center2) + (-0.5,-0.5,6)$);
      \coordinate (sbB) at ($(center2) + (-0.5,0.5,6)$);
      \coordinate (sbC) at ($(center2) + (0.5,0.5,6)$);
      \coordinate (sbD) at ($(center2) + (0.5,-0.5,6)$);
      \coordinate (sbA2) at ($(center2) + (-1,-1,8)$);
      \coordinate (sbB2) at ($(center2) + (-1,1,8)$);
      \coordinate (sbC2) at ($(center2) + (1,1,8)$);
      \coordinate (sbD2) at ($(center2) + (1,-1,8)$);
      \draw[cube] (sbA) -- (sbB) -- (sbC) -- (sbD) -- cycle;
      \draw[cube] (sbA2) -- (sbB2) -- (sbC2) -- (sbD2) -- cycle;
      \draw[cube] (sbA) -- (sbA2);
      \draw[cube] (sbB) -- (sbB2);
      \draw[cube] (sbC) -- (sbC2);
      \draw[cube] (sbD) -- (sbD2);


      \foreach \x in {-3,-1,...,3}
      \foreach \y in {-3,-1,...,3}
      {
        \draw[grid] (\x,-3,8) -- (\x,3,8);
        \draw[grid] (-3,\y,8) -- (3,\y,8);
      }
      \def\predsquare{(-3,-3,8)--(-3,3,8)--(3, 3, 8)--(3, -3, 8)--cycle}
      \begin{scope}
        \clip \predsquare;
        % the picture
        \draw[grid] (0,0,8) node[inner sep=0pt, opacity=0.65, cm={cos(\viewa),-sin(\viewa)*sin(\viewb), sin(\viewa),cos(\viewa)*sin(\viewb), (0,0)}] {\includegraphics[width=6cm]{tikz/map.jpg}};
      \end{scope}

      \draw[cube,->] (3.5,-3.5,0) node[below, scale=1.5]{$t$} -- (3.5,-3.5,8)node[above, scale=1.5]{$t+1$} ;
      % The arrow
      %\draw[ultra thick, ->, cm={cos(\viewa),-sin(\viewa)*sin(\viewb), sin(\viewa),cos(\viewa)*sin(\viewb), (0,0)}] (2,1,0) arc (-180:90:1cm);

\end{tikzpicture}
\caption{Architecture of the model v2}
\label{fig:arch3}
\end{figure}

